Tests as Maintainable Assets Via Auto-generated Spies: A case study involving the Scala collections library's Iterator trait

In testing stateful abstractions, it is often necessary to record interactions, such as method invocations, and express assertions over these interactions. Following the Test Spy design pattern, we can reify such interactions programmatically through additional mutable state. Alternatively, a mocking framework, such as Mockito, can automatically generate test spies that allow us to record the interactions and express our expectations in a declarative domain-specific language. According to our study of the test code for Scala's Iterator trait, the latter approach can lead to a significant reduction of test code complexity in terms of metrics such as code size (in some cases over 70% smaller), cyclomatic complexity, and amount of additional mutable state required. In this tools paper, we argue that the resulting test code is not only more maintainable, readable, and intentional, but also a better stylistic match for the Scala community than manually implemented, explicitly stateful test spies.

==> savedexcludedcontent.tex <==
% KL: saving all this content for a possible extended version of this report


% George; Tried using this to remove item spacing. But it's not having an effect. Some big object is 
% affecting constraints.

%\usepackage{enumitem}
%\setlist[itemize]{topsep=0pt}
%\usepackage{setspace}
%\titlespacing{\section}{0pt}{\parskip}{-\parskip}




%\todo[inline, color=red]{KL/GKT: abstract has 260w, need to cut down to about 100w once the intro stabilizes}

\todo[inline, color=red]{KL: George, you now have a bit more than one column for the intro, so I propose focusing on motivation and largely allowing background references to occur in the later sections}

\todo{GKT: To make actual writing possible and more distraction-free, I'm going to do a newpage temporarily and put the long todo items on that page.}


%\newpage


\todo[inline]{ALL: anticipate FAQs, e.g., what other mocking frameworks can I use}

\todo[inline]{ALL: double-check Scala examples against style guide}

%\todo[inline, color=red]{KL Tue 29 May 1) abstract DONE 2) object diagrams DONE 3) table of test methods 4) future work: static analysis tool for detecting smells, possibly based on supervised ML DONE}

\todo[inline]{KL: Scala 2.13 will have LazyList, which is lazy in head and tail, as opposed to Stream, which is lazy only in the tail and therefore doesn't rock.}

\todo[inline]{GKT: table showing use of scanLeft by GitHub org}

\todo[inline]{GKT: analyze use of scanLeft across major Scala projects -> motivation}

\todo[inline]{ALL: decide on final title}

% \todo[inline]{KL: review/fix line breaks}

\todo[inline, color=yellow]{KL Mon 21 May 08:30: 

- motivating context: big data in an IoT system such as home automation

- flesh out running example of two-stage pipeline: temp sensor | convert raw to degree C using map | compute cumulative (as opposed to sliding) running average using scanLeft

- complete imperative and functional examples

- long-running (indefinitely), regardless of data velocity (rate), need linear time, constant space

- correctness defined on finite prefixes -> opportunity to use property-based testing

- testing for simple overall result correctness vs. step-by-step incremental correctness of the interactions - effects of interactions with test result on original SUT: even though we are not allowed to interact directly with the SUT after using, say, scanLeft, the interactions with the test result are observable indirectly through the overall program behavior

- describe testing scenarios: 1) simple: instantiate SUT, invoke method, examine result; 2) incremental: instantiate SUT, invoke method, interact with result, examine effects on SUT (receiver of method)

- add diagrams for 2): object diagram to show how the SUT becomes a dependency of the result; sequence diagrams for map and scanLeft, where the first next() on the result DOES NOT trigger an invocation of next on the SUT

- add table for known examples including noExcessiveHasNextInJoinIterator: test code LOC w/o and w/ Mockito

- briefly discuss additional complexity in scenarios such as i1 ++ i2
}
%\todo[inline, color=red]{George: Shouldn't I be last author? I think you guys deserve to be first, given how much you've done already. Of course, I can amend this view if you are having me do more of the writing/editing, etc.}

%\todo[inline]{This is a tools paper from 2017, \url{https://dl.acm.org/citation.cfm?doid=3136000.3136012}}
%\todo[inline]{WONTFIX show sample build.sbt}
%\todo[inline]{DONE research how long the scanLeft bug has existed}
%\todo[inline]{DONE Comment from George: This comment is actually related to a long-standing interest of mine with the metrics project. We now have a way to analyze every line of code in a project--across all commits. If you can point me to the line number containing the bug (any commit is fine), I can probably identify how long this line has been in the code base. I suspect it has been there since scanLeft was introduced. Even if it is a group of lines, we can perform this analysis (perhaps with a bit of handwork).}
%\todo[inline]{DONE We should also investigate how long scanLeft has been tested. It would also be interested to know how many--if any--bug reports have ever been filed about it (open and closed). I'm guessing you investigated the latter carefully.}

% TODO John
% @Test def noExcessiveHasNextInJoinIterator: Unit = {

% DONE: look for venues
% https://conf.researchr.org/track/scala-2018/scala-2018-papers

% https://github.com/klaeufer/issue10709-scala
% https://github.com/scala/scala/blob/2.12.x/test/junit/scala/collection/IteratorTest.scala
% https://github.com/scala/scala/blob/v2.12.6/src/library/scala/collection/Iterator.scala#L604


%git clone -b 2.12.x --depth 1 git@github.com:scala/scala.git
%sbt test:compile % 5 min
%sbt test % Total time: 444 s

\todo[inline]{ideas:

- focus on software quality attributes of test suite by using a mock library instead of effectively doing the same thing manually

- explain significance to Scala community in terms of the practice of developing effective test suites

- think of test suites as assets

- TODO John: look at Iterator in depth

- TODO Konstantin: add a few spot examples from collection.mutable - look for cases of "manual mocking" to observe effects on dependencies (like in Iterator.scanLeft) - Stream, views (?) (these are similar to iterators), as well as other mutable collections and Observables

- next step: clone Scala 2.12.6 and manually review/mine the test suite for these classes
}

\todo[inline]{George: I've made some suggestions throughout.}

\todo[inline]{KL: talk about how the DSL allows the programmer clearly to convey intent}


%\newpage






\begin{abstract}
In this short experience paper, we study the effect of using automatically generated test spies on test code maintainability.
The software development community increasingly views automated tests as longer-term, maintainable assets along with the production code itself.
%Therefore, the community recognizes the importance of test code quality in terms of maintainability and related nonfunctional attributes.
In the context of our university-level programming languages class, we recently encountered a seven-year-old bug in the \texttt{scanLeft} method in the Scala collections library's \texttt{Iterator} trait, which includes some lazy stateful behaviors in its implementation that are challenging to test.
This motivated us to conduct a case study of this trait's test code and look for systematic ways to improve its maintainability. \todo{can we say robustness? Quality might be too strong a word here.}
Concretely, we have found that the test code includes several instances of manually implemented, explicitly stateful test spies, an approach we consider complex and error-prone. \todo{This sentence reads like an implementation detail. Move to main text? KL: directly tied to title, let's discuss}
According to our preliminary findings, using a mocking framework that supports automatically generated test spies as wrappers around existing objects, such as Mockito, can lead to a significant improvement of test code maintainability in terms of smaller size (in some cases up to 70\% less), readability, and conveying intent in terms of expressing expectations through a declarative domain-specific language.
We argue that this technique is of particular relevance to the Scala community because the resulting declarative test code is a better stylistic match for idiomatic Scala than manually implemented, explicitly stateful spies.
In addition, as our work is also education-facing, our hope is that this work helps to train the next generation of Scala developers how to write test code that is both comprehensible and maintainable. \todo{Agree?? had to eliminate "roboust" because it has a very specific meaning tied to fault tolerance}
\end{abstract}



\subsection*{Motivation}
\todo[inline]{These are all use cases. But you want to be clear what problem you want to solve. The above text is aimed at helping frame the general problem. Readers will only care about these examples if they understand the general nature of the problem first.}

\begin{itemize}
\item pipes and filters involving ongoing/indefinite/recurring computations, increasingly important for IoT
\item moving average example: imperative version
\item lazy structures to represent indefinite input/output
\item operations on lazy collections
\item moving average example: functional version using scanLeft
\item expected time and space complexity
\item expected interactive/incremental behavior (effects)
\end{itemize}



%\todo[inline]{KL: to save space, consider eliminating the first set of examples (temperature conversion)}


% \begin{figure*}
% \captionsetup{skip=\listingcaptionskip}
% \subfloat{\usebox{\TempConvImperative}}
% \hspace{\columnsep}
% \subfloat{\usebox{\TempConvFunctional}}
% \caption{Imperative and functional versions of the temperature conversion filter.}
% \label{fig:TempConvCode}
% \end{figure*}


% \begin{figure}
% \captionsetup{skip=\listingcaptionskip}
% \usebox{\TempConvOutput}
% \caption{Sample output of the temperature conversion filter.}
% \label{fig:TempConvOutput}
% \end{figure}



% \begin{figure*}
% \vspace*{\listingtopfigureskip}
% \captionsetup{skip=\listingcaptionskip}
% \captionsetup[subfloat]{captionskip=\listingsubcaptionskip}
% \subfloat[imperative version]{
% \usebox{\CumAvgImperative}
% \label{fig:CumAvgCodeImperative}
% }
% \hspace{\columnsep}
% \subfloat[functional version]{
% \usebox{\CumAvgFunctional}
% \label{fig:CumAvgCodeFunctional}
% }
% \caption{Imperative and functional versions of the cumulative running average filter. 
% Both run in linear time and constant space. 
% While the imperative version is monolithic, the functional version is a pipeline of consecutive modular, separately testable stages. 
% These latter qualities can lead to better maintainability and pedagogy.
% }
% \label{fig:CumAvgCode}
% \end{figure*}




For each value read, this program prints an updated cumulative running average.
Linear time/constant space but...besides the use of var, it is not modular, so not testable, not DRY.
Functional version with state encapsulated in the iterators; explain scanLeft and drop.


%
Must use iterator to stay in constant space!
Iterators also serve as clean interfaces between consecutive stages. 
Modular and testable (SUT is the line with scanLeft)! 
Shorter, less code duplication (print, read).

Cannot write this code using other methods, either: for comprehensions are based on map/flatMap, so they don't support any kind of accumulator. So we really need scanLeft to work properly.

Can write it using iterate/continually but need to lift into monad, e.g., Option, to handle termination.


\subsection*{Background, related work, definitions}
Talk about hidden vs. leaking state (state-based contracts, i.e., protocols): internal vs. external iterators 
\begin{itemize}
\item protocols
\item (cumulative) correctness
\item incremental (element-by-element) correctness
\item spy = partial mock
\end{itemize}

\cite{Bierhoff:2009:APC:1751509}

% https://stackoverflow.com/questions/18420995/scala-iterator-one-should-never-use-an-iterator-after-calling-a-method-on-it
% https://twitter.github.io/scala_school/specs.html
% https://stackoverflow.com/questions/12827580/mocking-vs-spying-in-mocking-frameworks
% https://stackoverflow.com/questions/4105592/comparison-between-mockito-vs-jmockit-why-is-mockito-voted-better-than-jmockit
% http://www.baeldung.com/mockito-vs-easymock-vs-jmockit


\todo[inline, color=red]{KL: remove/shorten any definitions George covers above - or vice versa}

\newpage














\todo[inline]{look for set of criteria for evaluating a technique}


scanLeft relatively unused internally


 Iterator, Stream, views (?)
 need inventory of methods returning a lazy collection along with their complexity and cumulative and element-by-element correctness (John is working on it


fail derministically on Linux with Java 8 and 10.
There appears to be nondeterminism on Linux with Java 9; 
see this build history for details: \url{https://travis-ci.org/klaeufer/mockito-spy-nondeterminism-scala/builds}.
Because Java 9 has reached EOL, we have replicated these experiments with Java 10 on Linux.


\begin{lstlisting}[style=lucscala]
@Test def testFrom(): Unit = {
  val it = spy(Iterator.from(1))
  verify(it, never).next()
}
\end{lstlisting}

\begin{lstlisting}[style=lucoutput]
[error] Test IteratorTest.testFrom failed: java.lang.NullPointerException: null, took 2.385 sec
[error]     at scala.collection.Iterator$$anon$8.next(Iterator.scala:159)
[error]     at scala.collection.Iterator$$anon$8.next(Iterator.scala:156)
[error]     at IteratorTest.testFrom(IteratorTest.scala:3)
\end{lstlisting}
Given that this exception occurs inside the 

\begin{lstlisting}[style=lucscala, firstnumber=156]
  def from(start: Int, step: Int): Iterator[Int] = new AbstractIterator[Int] {
    private var i = start
    def hasNext: Boolean = true
    def next(): Int = { val result = i; i += step; result }
  }
\end{lstlisting}




% https://travis-ci.org/klaeufer/mockito-issue-spy-scala

\begin{lstlisting}[style=lucoutput]
$ sbt test:dependencyTree
...
[info]   | 
[info]   +-org.mockito:mockito-inline:2.18.3
[info]     +-org.mockito:mockito-core:2.18.3
[info]       +-net.bytebuddy:byte-buddy-agent:1.8.5
[info]       +-net.bytebuddy:byte-buddy:1.8.5
[info]       +-org.objenesis:objenesis:2.6
\end{lstlisting}

% Java(TM) SE Runtime Environment (build 9+181)
% OSX Java 9 mockito-inline: PASS

% java version "1.8.0_172"
% OSX Java 8 mockito-inline: NPE

% java version "10.0.1" 2018-04-17
% Linux Java 10 mockito-core w/o resources: can't mock final
% Linux Java 10 mockito-core w/ resources: NPE
% Linux Java 10 mockito-inline: NPE

% java version "1.8.0_171"
% Linux Java 8 mockito-inline: NPE
% 

Java 10 on Linux:
\begin{lstlisting}[style=lucoutput]
[error] Test testAbstractIteratorPrivate failed
[error] Test testAbstractIteratorPrivateThis fai
[error] Test testFromPrivate failed
[debug] Test testIteratePrivateThis finished
[debug] Test testIteratorPrivate finished
[debug] Test testIteratorPrivateThis finished
\end{lstlisting}

Java 8 on Linux:
\begin{lstlisting}[style=lucoutput]
[error] Test testAbstractIteratorPrivate failed
[debug] Test testAbstractIteratorPrivateThis fin
[error] Test testFromPrivate failed
[debug] Test testIteratePrivateThis finished
[debug] Test testIteratorPrivate finished
[error] Test testIteratorPrivateThis failed
\end{lstlisting}


% \begin{itemize}
% \item static analysis tool for detecting smells, possibly based on supervised ML
% \item use repository mining to identify other projects that can benefit from this work
% \item systematic study of effect on nonfunctional quality metrics and process metrics (cite metrics dashboard paper)
% \item broader study across popular languages involving faculty and students
% \item how to measure sufficient test coverage in the presence of API protocols
% \item may be able to use property-based testing (ScalaCheck) more easily
% \end{itemize}

